Fighting Bias with Bias: Promoting Model Robustness by Amplifying Dataset Biases

NLP models often rely on superficial cues known as dataset biases to achieve impressive performance, and can fail on examples where these biases do not hold. Recent work sought to develop robust, unbiased models by filtering biased examples from training sets. In this work, we argue that such filtering can obscure the true capabilities of models to overcome biases, which might never be removed in full from the dataset. We suggest that in order to drive the development of models robust to subtle biases, dataset biases should be amplified in the training set. We introduce an evaluation framework defined by a bias-amplified training set and an anti-biased test set, both automatically extracted from existing datasets. Experiments across three notions of bias, four datasets and two models show that our framework is substantially more challenging for models than the original data splits, and even more challenging than hand-crafted challenge sets. Our evaluation framework can use any existing dataset, even those considered obsolete, to test model robustness. We hope our work will guide the development of robust models that do not rely on superficial biases and correlations. To this end, we publicly release our code and data.

==> tables/detailed_results.tex <==
\begin{table*}[]
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ll|cc|cc|cc@{}}
\toprule
\multicolumn{1}{c}{}               & \multicolumn{1}{c|}{}                           & \multicolumn{2}{c|}{MNLI} & \multicolumn{2}{c|}{ANLI} & \multicolumn{2}{c}{QQP}                 \\
\multicolumn{1}{c}{}               & \multicolumn{1}{c|}{}                           & Hard     & $\neg$ Hard    & Hard     & $\neg$ Hard    & Hard  & \multicolumn{1}{l}{$\neg$ Hard} \\ \midrule
\multirow{4}{*}{Data maps}         & $\mathcal{D}$                                   & 57.2     & 98.3           & 17.3     & 63.0           & 61.0  & 99.2                            \\
                                   & $\mathcal{D} \setminus \mathcal{D}_\text{hard}$ & 50.5     & 98.7           & 8.8      & 59.2           & 52.2  & 99.3                            \\
                                   & $\Delta$                                        & -6.6     & 0.4            & -8.6     & -3.8           & -8.8  & 0.1                             \\ \cmidrule(l){2-8} 
                                   & Size                                            & 1963     & 7852           & 640      & 2560           & 8086  & 32344                           \\ \midrule
\multirow{4}{*}{Partial-input}     & $\mathcal{D}$                                   & 77.8     & 92.9           & 31.9     & 60.9           & 78.9  & 95.1                            \\
                                   & $\mathcal{D} \setminus \mathcal{D}_\text{hard}$ & 67.7     & 93.5           & 18.6     & 62.3           & 58.9  & 95.7                            \\
                                   & $\Delta$                                        & -10.2    & 0.6            & -13.3    & 1.3            & -20.0 & 0.6                             \\ \cmidrule(l){2-8} 
                                   & Size                                            & 1963     & 7852           & 640      & 2560           & 8086  & 32344                           \\ \midrule
\multirow{4}{*}{Minority Examples} & $\mathcal{D}$                                   & 63.0     & 96.1           & 47.0     & 58.0           & 74.8  & 96.0                            \\
                                   & $\mathcal{D} \setminus \mathcal{D}_\text{hard}$ & 49.4     & 97.5           & 19.2     & 64.6           & 41.4  & 98.4                            \\
                                   & $\Delta$                                        & -13.6    & 1.4            & -27.8    & 6.6            & -33.3 & 2.4                             \\ \cmidrule(l){2-8} 
                                   & Size                                            & 1758     & 8057           & 924      & 2276           & 8086  & 32344                           \\ \bottomrule
\end{tabular}
\caption{\roberta-large models accuracy on held out instances in \mnli, per challenge set (cluster).}
\label{tab:mnli-detailed}
\end{table*}

==> tables/main_results_w_delta.tex <==
\begin{table*}[]
% \footnotesize
\centering
\resizebox{\textwidth}{!}{%

\begin{tabular}{@{}lllllllllllllllll@{}}
\toprule
 &
  \multicolumn{4}{c}{\mnli} &
  \multicolumn{4}{c}{\qqp} &
  \multicolumn{4}{c}{\wanli} &
  \multicolumn{4}{c}{\anli} \\
 &
  Val. &
  Hard-C &
  Hard-P &
  \multicolumn{1}{c|}{Hard-M} &
  Val. &
  Hard-C &
  Hard-P &
  \multicolumn{1}{c|}{Hard-M} &
  Val. &
  Hard-C &
  Hard-P &
  \multicolumn{1}{c|}{Hard-M} &
  Test &
  Hard-C &
  Hard-P &
  Hard-M \\ \midrule
100\% &
  $90.4_{0.2}$ &
  $59.9_{0.7}$ &
  $79.7_{0.6}$ &
  \multicolumn{1}{c|}{$71.9_{0.3}$} &
  $92.0_{0.1}$ &
  $59.4_{0.4}$ &
  $78.6_{0.2}$ &
  \multicolumn{1}{c|}{$73.5_{0.3}$} &
  $76.2_{0.1}$ &
  $19.7_{3.4}$ &
  $59.5_{0.6}$ &
  \multicolumn{1}{c|}{$60.2_{1.6}$} &
  $55.4_{0.1}$ &
  $14.8_{0.6}$ &
  $34.9_{1.0}$ &
  $44.3_{0.4}$ \\
random &
  $90.3_{0.1}$ &
  $59.5_{0.7}$ &
  $79.7_{0.7}$ &
  \multicolumn{1}{c|}{$71.9_{1.0}$} &
  $91.6_{0.1}$ &
  $57.8_{0.4}$ &
  $78.0_{0.5}$ &
  \multicolumn{1}{c|}{$71.8_{1.0}$} &
  $76.0_{0.1}$ &
  $17.6_{0.9}$ &
  $58.0_{3.0}$ &
  \multicolumn{1}{c|}{$59.2_{2.2}$} &
  $55.1_{0.7}$ &
  $15.7_{1.0}$ &
  $34.1_{1.4}$ &
  $44.2_{1.1}$ \\ \midrule
easy &
  $88.4^{\bigast}_{0.7}$ &
  $51.7_{0.5}$ &
  $68.2_{0.3}$ &
  \multicolumn{1}{c|}{$50.5_{1.2}$} &
  $88.3^{\bigast}_{1.9}$ &
  $49.0_{0.3}$ &
  $60.3_{1.8}$ &
  \multicolumn{1}{c|}{$31.3_{0.4}$} &
  $74.9^{\bigast}_{1.0}$ &
  $13.7_{0.8}$ &
  $43.5_{2.9}$ &
  \multicolumn{1}{c|}{$25.8_{2.4}$} &
  $51.2^{\bigast}_{1.9}$ &
  $5.8_{0.7}$ &
  $16.0_{1.0}$ &
  $12.3_{0.8}$ \\
\Delta &
  -2.0 &
  -8.2 &
  -11.5 &
  \multicolumn{1}{c|}{-21.4} &
  -3.7 &
  -10.4 &
  -18.3 &
  \multicolumn{1}{c|}{-42.2} &
  -1.3 &
  -6.0 &
  -16.0 &
  \multicolumn{1}{c|}{-34.4} &
  -4.2 &
  -9.0 &
  -18.9 &
  -32.0 \\ \bottomrule
\end{tabular}

}
\caption{Accuracy of \roberta-\modellarge models fine-tuned on different train splits of \mnli, \qqp, \wanli and \anli, and evaluated on the original and \hard test splits: dataset cartography (C), partial-input baselines (P) and minority examples (M). Reported values are averaged over 3 random seeds, with standard deviation as subscripts.
Results in the last row (\easy) are of training on one of the three \easy splits and testing on the respective \hard split, except for values  marked ($\bigast$) which are averaged over runs on all three \easy splits.
Model evaluation on bias-amplified splits results in weak performance on \hard test instances compared to the original data splits. 
} 
\label{tab:main_results}
\end{table*}

==> tables/sanity_minority.tex <==

% on roberta-large
\begin{table}[]
\footnotesize
\centering
\resizebox{\columnwidth}{!}{%


\begin{tabular}{@{}llccl@{}}
\toprule
                       &             & \multicolumn{3}{c}{Test Data}                                                      \\ \cmidrule(l){3-5} 
                       &             & All                              & Easy                             & Hard         \\ \midrule
\multirow{2}{*}{\mnli} & 100\% train & $90.4_{0.2}$                     & $95.3_{0.2}$                     & $71.9_{0.3}$ \\
                       & easy        & $87.6_{0.2}$                     & $97.4_{0.2}$                     & $50.5_{1.2}$ \\ \midrule
\multirow{2}{*}{\qqp}  & 100\% train & $92.0_{0.1}$                     & $96.2_{0.0}$                     & $73.5_{0.3}$ \\
                       & easy        & $85.9_{0.0}$                     & $98.3_{0.1}$                     & $31.3_{0.4}$ \\ \midrule
\multirow{2}{*}{\wanli} & 100\% train & \multicolumn{1}{l}{$76.2_{0.1}$} & \multicolumn{1}{l}{$78.5_{0.3}$} & $60.2_{1.6}$ \\
                       & easy        & \multicolumn{1}{l}{$73.7_{0.3}$} & \multicolumn{1}{l}{$80.7_{0.2}$} & $25.8_{2.4}$ \\ \midrule
\multirow{2}{*}{\anli}  & 100\% train & \multicolumn{1}{l}{$55.4_{0.1}$} & \multicolumn{1}{l}{$59.9_{0.1}$} & $44.3_{0.4}$ \\
                       & easy        & \multicolumn{1}{l}{$50.2_{0.3}$} & \multicolumn{1}{l}{$66.0_{0.2}$} & $12.3_{0.8}$ \\ \bottomrule
\end{tabular}


}



\caption{.}
\label{tab:sanity_partial}
\end{table}

==> tables/sanity_partial_input.tex <==

% on deberta-large
\begin{table}[!t]
\footnotesize
\centering
\resizebox{\columnwidth}{!}{%


\begin{tabular}{@{}llccl@{}}
\toprule
                       &             & \multicolumn{3}{c}{Test Data}                                                      \\ \cmidrule(l){3-5} 
                       &             & All                              & Easy                             & Hard         \\ \midrule
\multirow{2}{*}{\mnli} & 100\% train & $91.1_{0.1}$                     & $93.7_{0.2}$                     & $81.4_{0.3}$ \\
                       & easy        & $89.6_{0.1}$                     & $94.3_{0.1}$                     & $71.8_{0.5}$ \\ \midrule
\multirow{2}{*}{\qqp}  & 100\% train & $93.0_{0.0}$                     & $95.6_{0.1}$                     & $81.3_{0.1}$ \\
                       & easy        & $90.3_{0.2}$                     & $96.1_{0.1}$                     & $63.9_{0.3}$ \\ \midrule
\multirow{2}{*}{\wanli} & 100\% train & \multicolumn{1}{l}{$77.1_{0.5}$} & \multicolumn{1}{l}{$79.3_{0.4}$} & $62.6_{2.0}$ \\
                       & easy        & \multicolumn{1}{l}{$76.7_{0.1}$} & \multicolumn{1}{l}{$80.8_{0.1}$} & $49.6_{1.0}$ \\ \midrule
\multirow{2}{*}{\anli}  & 100\% train & \multicolumn{1}{l}{$67.5_{0.5}$} & \multicolumn{1}{l}{$71.3_{0.5}$} & $50.0_{0.6}$ \\
                       & easy        & \multicolumn{1}{l}{$63.2_{0.4}$} & \multicolumn{1}{l}{$70.8_{0.2}$} & $28.3_{1.3}$ \\ \bottomrule
\end{tabular}


}



\caption{Accuracy of \deberta-\modellarge models fine-tuned on the \easy and 100\% train splits of \mnli, \qqp, \wanli and \anli, and evaluated on \hard, \easy and \emph{all} instances of the test set; \easy and \hard splits are based on the \partialinput method.
When training in a bias-amplified setting, performance on the full test set slightly decreases due to large drops on \hard test instances, while performance on \easy test instances is generally unaffected.
}
\label{tab:sanity_partial}
\end{table}
